Rough-Terrain Locomotion and Unilateral Contact Force Regulations With a Multi-Modal Legged Robot

Despite many accomplishments by legged robot designers, state-of-the-art bipedal robots are prone to falling over, cannot negotiate extremely rough terrains and cannot directly regulate unilateral contact forces. Our objective is to integrate merits of legged and aerial robots in a single platform. We will show that the thrusters in a bipedal legged robot called Harpy can be leveraged to stabilize the robot's frontal dynamics and permit jumping over large obstacles which is an unusual capability not reported before. In addition, we will capitalize on the thrusters action in Harpy and will show that one can avoid using costly optimization-based schemes by directly regulating contact forces using an Reference Governor (RGs). We will resolve gait parameters and re-plan them during gait cycles by only assuming well-tuned supervisory controllers. Then, we will focus on RG-based fine-tuning of the joints desired trajectories to satisfy unilateral contact force constraints.

==> old_contents.tex <==

% OLD CONTENT (Kaier's)
\begin{comment}





\begin{equation}
  \bm{p}_{P} = \bm{P}_{B} + R_{B}\, \bm{l}_{1}^{B}
  \end{equation}
  
 \begin{equation}
  \boldsymbol{P}_{H}=\boldsymbol{P}_{p}+R_{B} R_{x}\left(\phi_{F}\right) \boldsymbol{l}_{2}^{P}
\end{equation}

\begin{equation}
\boldsymbol{P}_{K}=\boldsymbol{P}_{H}+R_{B} R_{x}\left(\phi_{F}\right) R_{y}\left(\phi_{S}\right) \boldsymbol{l}_{3}^{H}
\end{equation}

\begin{equation}\boldsymbol{P}_{F}=\boldsymbol{P}_{K}+R_{B} R_{x}\left(\phi_{F}\right) R_{y}\left(\phi_{S}\right) R_{y}\left(\gamma_{S}\right) \boldsymbol{l}_{4}^{K}
\end{equation}

\begin{equation}
\boldsymbol{P}_{T}=\boldsymbol{P}_{B}+R_{B} \boldsymbol{\ell}_{t}^{B}
\end{equation}
%
where $\boldsymbol{P}$ is position vector, subscripts denote body, pelvis, hip, knee, foot and thruster. $R$ is rotation matrix and the subscripts denote different reference frames. $\phi_F,\phi_S,\gamma_F,$ denote the hip front, hip sagittal and knee sagittal angles respectively for the left and right foot. $\boldsymbol{l}_1^B$, $\boldsymbol{l}_2^P$, $\boldsymbol{l}_3^H$, $\boldsymbol{l}_T^B$and are constant. $\boldsymbol{l}_4^K$, position vector from knee to foot, can be derived as
\begin{equation}\boldsymbol{l}_{4}^{k}=\left[\begin{array}{cc}
-L_{4 a}-L_{4 b}\sin \gamma_{s} \\
0 \\
-L_{4 b} \cos \gamma_{s}
\end{array}\right]\end{equation}\\
where $L_{4a}$ and $L_{4b}$ are both constant, and positions on the other side leg have similar derivation.

Here angular velocity are only considered for body and actuators.
\begin{equation}
    \boldsymbol{\omega}_H^B = \left[\begin{array}{l}
\dot{\phi}_{F} \\
0 \\
0
\end{array}\right]+\boldsymbol{\omega}_{B}^{B}
\end{equation}

\begin{equation}
    \boldsymbol{\omega}_K^B = \left[\begin{array}{l}
\dot{\phi}_{S} \\
0 \\
0
\end{array}\right]+\boldsymbol{\omega}_{B}^{B}
\end{equation}
where $\boldsymbol{\omega}_{B}^{B}$ is the body angular velocity.\\

\par The full dynamics of Harpy model is derived using Euler-Lagrange equation.The kinetic energy of the body is
\begin{equation}K=\sum_{F \in \mathcal{F}}\left(\frac{1}{2} m_{F} \boldsymbol{\dot P}_F^T \boldsymbol{P}_{F}+\frac{1}{2} \boldsymbol{\omega}_{F}^{FT}I_{F} \boldsymbol{\omega}_{F}^{F}\right)\end{equation}
and the potential energy is
\begin{equation}V=-\sum_{F \in \mathcal{F}} m_{F} \boldsymbol{P}_{F}^T\left[\begin{array}{c}
0 \\
0 \\
-g
\end{array}\right]\end{equation}
 \begin{equation}
 \mathcal{F}=\left\{B, H_{L}, K_{L}, H_{R}, K_{R}\right\}
 \end{equation}
 
 
  kinematic of knee angle is
 \begin{equation}\boldsymbol{\gamma}=\left[\begin{array}{l}
\gamma_{s,L} \\
\gamma_{s,R}
\end{array}\right]\end{equation}
\begin{equation}\ddot{\boldsymbol{\gamma}}=\boldsymbol{u}_{\gamma}\end{equation}
 
 
 
 $\boldsymbol{\omega}_B^B$ uses modified Lagrangian
\begin{equation}\dot{R}_{B}=R_{B}\left[\boldsymbol{\omega}_{B}\right]_{x}\end{equation}
\begin{equation}\frac{d}{d t}\left(\frac{\partial L}{\partial \boldsymbol{w}_{B}^{B}}\right)+\boldsymbol{w}_{B}^{B} \times \frac{\partial L}{\partial \boldsymbol{\omega}_{B}^{B}}+\sum_{j=1}^{3} \boldsymbol{r}_{Bj} \times \frac{\partial L}{\partial \boldsymbol{r}_{B j}}=\boldsymbol{\tau}_{B}^{B}\end{equation}

Where $\left[\cdot\right]_x$ is skew operator. Forming the Lagrangian $L = K - V$ for the rest of state:
\begin{equation}\frac{d}{d t}\left(\frac{\partial L}{\partial \boldsymbol{\dot{q}}}\right)-\frac{\partial L}{\partial \boldsymbol{q}}=\boldsymbol{u}\end{equation}

\begin{equation}\boldsymbol{q}=\left[\begin{array}{c}
\boldsymbol{P}_{B} \\
\boldsymbol{\theta}_{L} \\
\boldsymbol{\theta}_{R}
\end{array}\right],\quad
\boldsymbol{\theta_{L}}=\left[\begin{array}{l}
\phi_{F,L} \\
\phi_{S,L}
\end{array}\right], \quad \boldsymbol{\theta}_{R}=\left[\begin{array}{l}
\phi_{F,R} \\
\phi_{S,R}
\end{array}\right]\end{equation}
 
 This forms the standard acceleration form
\begin{equation}M\left[\begin{array}{c}
\boldsymbol{\dot{\omega}}_{B}^{B} \\
\boldsymbol{\ddot{q}} \\
\boldsymbol{\ddot{\gamma}}
\end{array}\right] + \boldsymbol{h} =  B_{m} \boldsymbol{u}_{m}+B_{t} \boldsymbol{u}_{t}+B_g \boldsymbol{u}_g
\end{equation}

\begin{equation}B_{m}=\left[\begin{array}{c}
O_{6 \times 6} \\
I_{6 \times 6}
\end{array}\right], \quad \boldsymbol{u}_{m}=\left[\begin{array}{c}
\boldsymbol{u}_{q} \\
\boldsymbol{u}_{\gamma}
\end{array}\right]\end{equation}

\begin{equation}B_t = \left[\begin{array}{c}
\left(\begin{array}{c}
\frac{\partial \boldsymbol{p}_{T,L}}{\partial \hat{z}} \\
\frac{\partial \boldsymbol{p}_{T,R}}{\partial \boldsymbol{z}}
\end{array}\right)^T\\
O_{2 \times 6}\end{array}\right], \quad
\boldsymbol{u}_{t}=\left[\begin{array}{l}
\boldsymbol{u}_{t,L} \\
\boldsymbol{u}_{t,R}
\end{array}\right]
\end{equation}

\begin{equation}B_t = \left[\begin{array}{c}
\left(\begin{array}{c}
\frac{\partial \boldsymbol{p}_{F,L}}{\partial \boldsymbol{z}} \\
\frac{\partial \boldsymbol{p}_{F,R}}{\partial \boldsymbol{z}}
\end{array}\right)^T\\
O_{2 \times 6}\end{array}\right], \quad
\boldsymbol{u}_{g}=\left[\begin{array}{l}
\boldsymbol{u}_{g,L} \\
\boldsymbol{u}_{g,R}
\end{array}\right]
\end{equation}

\begin{equation}\boldsymbol{z}=\left[\begin{array}{c}
\omega_{B}^{B} \\
\dot{q}
\end{array}\right]_{10 \times 1}\end{equation}

Where $\boldsymbol{u}_{m}$,$ \boldsymbol{u}_{t}$ and $ \boldsymbol{u}_g$ represent the joint actuators, thrusters and ground actions respectively.

\par The full model is written in state space form 
\begin{equation}
\bm{\dot x} = f(\bm{x},\bm{u}_{m},\bm{u}_{t},\bm{u}_{g})
\end{equation}
and system state are defined as 
\begin{equation}
\boldsymbol{x}=\left[\boldsymbol{r}_B; \boldsymbol{q};\boldsymbol{\gamma}; \boldsymbol{\omega}_B;  \boldsymbol{\dot q};\boldsymbol{\dot \gamma}\right];
\end{equation}\\
 



\par The system uses compliant ground model
\begin{equation}\boldsymbol{u}_{g,L}=\left[\begin{array}{c}
f_{x_{L}} \\
f_{y_{L}} \\
f_{z_{L}}
\end{array}\right]
\end{equation}
\begin{equation}f_{z}=\left\{\begin{array}{l}
-k_{pg} p_{F,z}-k_{dg} \dot{p}_{f,z},\null\hfill \text { if } P_{F,z}<0, P_{F,z}<0 \\
-k_{pg} p_{F,z}, \null\hfill \text { if } P_{F,z}<0, \dot{P}_{F,z} \geqslant 0 \\
0 \null\hfill \text{else}
\end{array}\right.\end{equation}

\begin{equation}f_x=\left\{\begin{array}{l}
-\left(\mu_{c}+\left(\mu_{s}-\mu_{c}\right) e^{-\frac{\left|P_{F x}\right|^{2}}{v_{s}^{2}}}\right) f_{z} \cdot \operatorname{sign}\left(\dot{p}_{F,x}\right)-\mu_{v} \dot{p}_{F,x} \\
0
\end{array}\right.\end{equation}
where $v_s$ is stribeck velocity, $\mu_s$, $\mu_c$ and $\mu_v$ are static, coulomb and viscous friction coefficients respectively.


The ODE is numerically approximated by fourth-order Runge-Kutta methods.






%
\begin{equation}B(t)=\sum_{i=0}^{4}\left(\begin{array}{l}
4 \\
i
\end{array}\right) P_i(1-s)^{4-i} s^{i}\end{equation}
Where $s = \frac{mod(t,0.75)}{0.75}$, $P_0$ is the starting point of Bezier curve, $P_2$ is the midpoint of Bezier curve and $P_4$ is the end point of Bezier curve. Defining $P_1 = P_0$ and $P_4 = P_3$ for zero velocity constrain at start and end positions. Free parameters $P_0,P_2,P_4$ with the initial orientation and velocity of the body are founded by optimization.
\par The dynamics of the constrained model can be derived as.
\begin{equation}\left[\begin{array}{cc}
\boldsymbol{M} & -\boldsymbol{J}_{s}^{\top} \\
\boldsymbol{J}_{s} & \boldsymbol{O}_{3\times 3}
\end{array}\right]\left[\begin{array}{l}
\boldsymbol{\dot q} \\
\boldsymbol{\lambda}
\end{array}\right]=\left[\begin{array}{l}
\boldsymbol{h}_{0} \\
\boldsymbol{O}_{3 \times 1}
\end{array}\right]\end{equation} 
%
where $\boldsymbol{M}$ is the diagnal mass matrix, $\boldsymbol{h}_0 = -\boldsymbol{h} + B_m \boldsymbol{u}_m + B_g \boldsymbol{u}_g$. $\boldsymbol{J}_s$ is the constraint matrix to constraint the motion in y direction and roll and yaw. $\boldsymbol{\lambda}$ is the Lagrangian multiplier, and $\boldsymbol{J}_{s}^{\top} \boldsymbol{\lambda}$ represents the constraint forces. 


\par The bezier parameters founded through optimization form swing and stance curves which are assigned to left and right legs alternatively for successive walking gait along with the initial condition of the body center of mass.


\section{Gait design}
\label{sec:gait_controller}

\textcolor{blue}{
This section contains the gait design and the controller action for assisting the walking and jumping. 
\begin{itemize}
    \item Walking gait optimization using 2D constrained model.
    \item Design of the center of mass trajectory to avoid obstacle.
    \item Using thrusters to stabilize roll-yaw motions for walking using the 2D gait, and track target body center of mass trajectory.
    \item ERG. $\theta$
\end{itemize}
}

% ----------------------------------------------------------
\subsection{Walking gait design}

\textcolor{blue}{
\begin{itemize}
    \item Define the Bezier curve for the walking gait.
    \item Define the Lagrange multiplier constraint for the 2D walking gait.
    \item Optimization problem for finding the gait.
\end{itemize}
}


% ----------------------------------------------------------
\subsection{Trajectory for avoiding obstacles}

\textcolor{blue}{
\begin{itemize}
    \item Manually setup? Just show the equations of the trajectory.
\end{itemize}
}




% ----------------------------------------------------------
\subsection{Joint and thruster controller}

\textcolor{blue}{
\begin{itemize}
    \item PID and PD controller. If too short, this can be put in the previous section.
\end{itemize}
}
\par Controller for the joints actions in walking gait are designed to track the footstep founded in the previous bezier polynomial using PID controller. 




% \begin{figure}[t]
%     \vspace{0.05 in}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/harpy_controller.eps}
%     \caption{The controller design of Harpy, where $r,x$ and $u$ denotes the state references, state and control signal. Superscript * denotes control signals, states and references for MPC and $'$ for normal (PD or PID) control}
%     \label{fig:controller}
%     \vspace{-0.05in}
% \end{figure}

subject to the state model and constraints: 
%
\begin{equation}
\begin{aligned}
    \dot{\bm x}_{dp} &= f(\bm x_{dp},\bm u_{dp}), &
    q_{ref}^{j+1} &= \theta^j + q_c \\
    \boldsymbol{p}_{Bt}^{j+1} &= h(\bm p_{Bt}^j,t), &
    \left|\boldsymbol{u}_{dp}\right|  &\leq \boldsymbol{u}_{dp\max }
\end{aligned}
\label{eq:model_vlip_constraint}
\end{equation}









{\color{red}I recommend you wrap all constraints, cost functions, etc., as form like this:

\[
\min _{x(-), u(\cdot), p, t_{i}} \int_{0}^{t_{f}} \Phi_{L}(t, x(t), u(t), p) d t+\Phi_{M}\left(t_{f}\right)
\]
subject to:
\[
\begin{aligned}
\dot{x}(t) &=f_{i}(t, x(t), u(t), p) \\
x\left(t_{i+1}^{+}\right) &=h_{i}\left(x\left(t_{i}^{-}\right), p\right) \\
g_{i}(t, x(t), u(t), p) & \geq 0 \\
r^{e q}\left(x(0), \ldots, x\left(t_{f}\right), p\right) &=0 \\
r^{\text {ineq}}\left(x(0), \ldots, x\left(t_{f}\right), p\right) & \geq 0
\end{aligned}
\]

Then, spend some paragraphs to explain your MPC problem. Squeeze all Eqs. 14-19 inside above equation as well.} 





A double support standing step is added before the jumping to reset the initial position $\bm p_{Bt}^0$ to be the standing position. The MPC is used for achieving proper leg position and body posture at landing time thus allowing smooth transition from landing to walking. Therefore, $\bm q_c$, a constant value of $\bm q$ depending on the desired landing posture is included in the reference function along with the current body pitch $\theta^j$. This reference can ensure the legs do not lag behind the body at landing time, and $\bm q_c$ can be properly adjusted to achieve desired landing posture. 

The MPC runs at a much lower frequency than the full model, and uses zero order hold for generated control signal $u_{dp}$ which is directly applied to the  full model while the rest of control signals use PID or PD control.  



\end{comment}
